Interaction Modeling with Multiplex Attention

Modeling multi-agent systems requires understanding how agents interact. Such systems are often difficult to model because they can involve a variety of types of interactions that layer together to drive rich social behavioral dynamics. Here we introduce a method for accurately modeling multi-agent systems. We present Interaction Modeling with Multiplex Attention (IMMA), a forward prediction model that uses a multiplex latent graph to represent multiple independent types of interactions and attention to account for relations of different strengths. We also introduce Progressive Layer Training, a training strategy for this architecture. We show that our approach outperforms state-of-the-art models in trajectory forecasting and relation inference, spanning three multi-agent scenarios: social navigation, cooperative task achievement, and team sports. We further demonstrate that our approach can improve zero-shot generalization and allows us to probe how different interactions impact agent behavior.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
 \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
  \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{\href{https://github.com/fanyun-sun/IMMA}{Click here for Code.}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section 4 and the Appendix.}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
  \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See the Appendix.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See the Appendix.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Refer to \href{https://github.com/fanyun-sun/IMMA}{this repository}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We only used public benchmark datasets and synthetic datasets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
   \answerNA{}
\end{enumerate}

\end{enumerate}


==> tables/bball_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!tbp]
\vspace{-3mm}
\caption{Trajectory prediction results on the NBA dataset.}
\vspace{-2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\toprule
\midrule
\multirow{2}{*}{Metrics} & \multicolumn{6}{c|}{Baseline Methods}  & \multicolumn{3}{c}{\method{}}      \\ 
\cmidrule{2-10}
                & \multicolumn{1}{c|}{MLP} & \multicolumn{1}{c|}{GAT\_LSTM~\citep{velivckovic2017graph}}  & \multicolumn{1}{c|}{NRI~\citep{kipf2018neural}} & \multicolumn{1}{c|}{EvolveGraph~\citep{li2020evolvegraph}} & \multicolumn{1}{c|}{RFM (skip 1)} & \multicolumn{1}{c|}{RFM~\citep{tacchetti2018relational}} & \multicolumn{1}{c|}{SG} & \multicolumn{1}{c|}{MG} & 
                \multicolumn{1}{c}{MG + PLT}\\ 
                         \midrule
                         
ADE $\downarrow$ & 1.113 $\pm$ 0.002  & 0.978 $\pm$ 0.005  & 0.946 $\pm$ 0.005 & 0.896 $\pm$ 0.009 & 0.938 $\pm$ 0.003  & 0.839 $\pm$ 0.020  & 0.860 $\pm$ 0.008  & 0.833 $\pm$ 0.017  & \textbf{0.769 $\pm$ 0.009} \\
FDE $\downarrow$ & 1.990 $\pm$ 0.002  & 1.733 $\pm$ 0.010  & 1.818 $\pm$ 0.017 & 1.695 $\pm$ 0.016 & 1.756 $\pm$ 0.005  & 1.572 $\pm$ 0.034  & 1.612 $\pm$ 0.015  & 1.562 $\pm$ 0.027  & \textbf{1.438 $\pm$ 0.019}    \\ %\hline
%$\text{minADE}_{10}$            &&&&&&&&& \\
%$\text{minFDE}_{10}$            &&&&&&&&&  \\
%\midrule
%Graph Acc (\%) & \text{nan} & 55.34  & 71.90 &   &&& 82.58 &  \\
\bottomrule
\end{tabular}
}
\label{tab:bball}
\end{table*}

==> tables/lf_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\newpage
\begin{table*}[!tbp]
\caption{Trajectory prediction results on the Social Navigation Environment.}% \jw{It'd be good to cite the baselines ideally in the table but at least in the caption.}}
\vspace{-2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\toprule
\midrule
\multirow{2}{*}{Metrics} & \multicolumn{6}{c|}{Baseline Methods}  & \multicolumn{3}{c}{\method{} (ours)}      \\ 
\cmidrule{2-10}
                & \multicolumn{1}{c|}{MLP} & \multicolumn{1}{c|}{GAT\_LSTM~\citep{velivckovic2017graph}}  & \multicolumn{1}{c|}{NRI~\citep{kipf2018neural}} & \multicolumn{1}{c|}{EvolveGraph~\citep{li2020evolvegraph}} & \multicolumn{1}{c|}{RFM (skip 1)} & \multicolumn{1}{c|}{RFM~\citep{tacchetti2018relational}} & \multicolumn{1}{c|}{SG} & \multicolumn{1}{c|}{MG} & 
                \multicolumn{1}{c}{MG + PLT} \\ 
                         \midrule
ADE $\downarrow$             & 0.241 $\pm$ 0.006  & 0.306 $\pm$ 0.008  & 0.217 $\pm$ 0.005 & 0.160 $\pm$ 0.003 &  0.160 $\pm$ 0.002  & 0.156 $\pm$ 0.003  & 0.164 $\pm$ 0.002  & 0.148 $\pm$ 0.004  & \textbf{0.139 $\pm$ 0.001} \\
FDE $\downarrow$           & 0.513 $\pm$ 0.012  & 0.527 $\pm$ 0.009  & 0.386 $\pm$ 0.009 & 0.321 $\pm$ 0.006 & 0.325 $\pm$ 0.004  & 0.317 $\pm$ 0.005  & 0.327 $\pm$ 0.003  & 0.294 $\pm$ 0.006  & \textbf{0.279 $\pm$ 0.002} \\
%\midrule
%Graph Acc. (\%) $\uparrow$ & \text{-} & 21.83 $\pm$ 0.67  & 57.18 $\pm$ 0.14 & 70.23 $\pm$ 0.36 & 70.05 $\pm$ 0.55  & 71.53 $\pm$ 0.56  & \textbf{80.15 $\pm$ 1.48}  & 77.98 $\pm$ 0.16  & \textbf{81.38 $\pm$ 0.29} \\
\bottomrule
\end{tabular}
}
\label{table:lf_results}
\end{table*}



==> tables/phase_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\newpage
\begin{table*}[!tbp]
\vspace{-3mm}
\caption{Trajectory prediction results on PHASE dataset.}
\vspace{-2mm}
\label{tab:phase}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\toprule
\midrule
\multirow{2}{*}{Metrics} & \multicolumn{6}{c|}{Baseline Methods}  & \multicolumn{3}{c}{\method{}}      \\ 
\cmidrule{2-10}
                & \multicolumn{1}{c|}{MLP} & \multicolumn{1}{c|}{GAT\_LSTM~\citep{velivckovic2017graph}}  & \multicolumn{1}{c|}{NRI~\citep{kipf2018neural}} & \multicolumn{1}{c|}{EvolveGraph~\citep{li2020evolvegraph}} & \multicolumn{1}{c|}{RFM (skip 1)} & \multicolumn{1}{c|}{RFM~\citep{tacchetti2018relational}} & \multicolumn{1}{c|}{SG} & \multicolumn{1}{c|}{MG} & 
                \multicolumn{1}{c}{MG + PLT} \\ 
                         \midrule
ADE $\downarrow$ & 1.024 $\pm$ 0.005  & 1.545 $\pm$ 0.040  & 0.986 $\pm$ 0.011 & 0.848 $\pm$ 0.012 & 0.870 $\pm$ 0.008  & 0.892 $\pm$ 0.008  & 0.875 $\pm$ 0.020  & 0.883 $\pm$ 0.024   & \textbf{0.801 $\pm$ 0.009} \\
FDE $\downarrow$ & 1.763 $\pm$ 0.024  & 2.527 $\pm$ 0.063  & 1.772 $\pm$ 0.024  & 1.522 $\pm$ 0.019 & 1.581 $\pm$ 0.030  & 1.630 $\pm$ 0.042  & 1.585 $\pm$ 0.044  & 1.593 $\pm$ 0.048   & \textbf{1.484 $\pm$ 0.014} \\
%\midrule
%Graph Acc. (\%) $\uparrow$ & \text{-} & 52.94 $\pm$ 1.66  & 55.30 $\pm$ 2.09 & 58.96 $\pm$ 1.31 & 55.30 $\pm$ 2.09  & 54.71 $\pm$ 0.83  & \textbf{78.82 $\pm$ 3.54}  & \textbf{79.02 $\pm$ 4.04} & \textbf{79.21 $\pm$ 1.42}  \\
\bottomrule
\end{tabular}
}
%\vspace{-1cm}
\end{table*}


